$\textit{Jump Your Steps}$: Optimizing Sampling Schedule of Discrete Diffusion Models

Diffusion models have seen notable success in continuous domains, leading to the development of discrete diffusion models (DDMs) for discrete variables. Despite recent advances, DDMs face the challenge of slow sampling speeds. While parallel sampling methods like $\tau$-leaping accelerate this process, they introduce $\textit{Compounding Decoding Error}$ (CDE), where discrepancies arise between the true distribution and the approximation from parallel token generation, leading to degraded sample quality. In this work, we present $\textit{Jump Your Steps}$ (JYS), a novel approach that optimizes the allocation of discrete sampling timesteps by minimizing CDE without extra computational cost. More precisely, we derive a practical upper bound on CDE and propose an efficient algorithm for searching for the optimal sampling schedule. Extensive experiments across image, music, and text generation show that JYS significantly improves sampling quality, establishing it as a versatile framework for enhancing DDM performance for fast sampling.

==> 3method.tex <==
\section{Optimizing the sampling schedule of discrete diffusion models}

In this section, our objective is to find an optimal sampling schedule \((T, t_1, \dots, t_n, 0)\) that minimizes the \textit{compounding decoding error} (CDE) caused by parallel sampling. In Section 3.1, we define and analyze the CDE, providing an intuitive understanding of how the sampling schedule is related to it. Next, we derive an upper bound on the CDE induced by parallel sampling (Section 3.2) and introduce techniques to compute the upper bound tractable and applicable for sampling schedule optimization (Section 3.3). Finally, in Section 3.4, we propose a hierarchical breakdown strategy that finds the optimal sampling schedule by decomposing a coarse schedule into finer steps. Although this section focuses on samplers based on \(\tau\)-leaping, all methods are also applicable to the \(k\)-Gillespie algorithm. For extensions to \(k\)-Gillespie, please refer to the Appendix.

% In this section, our objective is to find optimal sampling schedule \((T, t_1, \dots, t_n, 0)\) that minimize the \textit{compounding decoding error} (CDE) caused by parallel sampling. In Section 3.1, we define and analyze CDE and provide an intuitive explanation of how sampling schedule is related to CDE. Next, we formulate the upper bound of CDE induced by parallel sampling (Section 3.2) and introduce techniques that make the computation tractable and applicable to sampling schedule optimization (Section 3.3). Finally, in Section 3.4, we propose a hierarchical breakdown strategy that finds the optimal sampling schedule by decomposing the coarse sampling schedule into finer steps. Although this section focuses on sampler based on \(\tau\)-leaping, all methods are also applicable to \(k\)-Gillespie. For extensions to \(k\)-Gillespie, please refer to the Appendix.

\subsection{Motivating Examples: The Time-Dependent Nature of Compounding Errors}

Before formally introducing our method, we begin with a simple analysis to illustrate why an improved sampling schedule can reduce the compounding error. Recall that the compounding error denotes the mismatch between the true joint distribution and the distribution resulting from the parallel generation of different tokens. The compounding error can be quantified using the KL divergence between the joint distribution \( P_{X,Y} \) and the product of the marginal distributions \( P_X \otimes P_Y \), where \( X \) and \( Y \) refer to different tokens:

\begin{equation}
\text{Compounding Error} 
\triangleq D_{\mathrm{KL}}(
\underbrace{P_{X,Y}}_{\textrm{True distribution}} 
\| 
\underbrace{P_X \otimes P_Y }_{\textrm{Approx.\ distribution}} 
) 
= I(X; Y)
\label{equation:CDE}
\end{equation}



\begin{equation}
\text{Compounding Error of }  \mathbf{X}_t 
\triangleq D_{\mathrm{KL}}(
\underbrace{q_t(\mathbf{X}_t)}_{\textrm{True distribution}} 
\| 
\underbrace{P_{x_t^{(1)}} \otimes P_{x_t^{(2)}} \otimes\cdots \otimes P_{x_t^{(S)}}}_{\textrm{\jc{Approx.\ distribution with parallel sampling}}} 
) 
=?? I((x_t^{(i)})_{i=1,\cdots,S}),
\label{equation:CDE}
\end{equation}
where $\mathbf{X}_t = (x_t^{(i)})_{i=1,\cdots,S}$

Want to say: 
$I\Big((x_t^{(i)})_{i=1,\cdots,S}\Big) \geq I\Big((x_t^{(i)})_{i=1,\cdots,S} | (x_t^{(i_k)})_{i_k \in\{1,\cdots,S\}} \Big)$

where \( I(X; Y) \) denotes the mutual information between \( X \) and \( Y \). This expression shows that the compounding error is directly related to the mutual information between the tokens; the smaller the mutual information, the less error is introduced by parallel sampling.

\begin{wrapfigure}{r}{6cm}
\includegraphics[width=5cm]{figures-png/MI.png}
\caption{
    \textbf{MI.}
    MI.
}
\label{homogenity-sample}
\end{wrapfigure}

Our key intuition is that when we sample sequences using discrete diffusion models (DDMs), the mutual information between tokens evolves over time, leading to variations in the compounding error at different timesteps. For example, consider generating text using masked DDMs. In the early stages of generation (those close to \( T \)), the mutual information between tokens \( I(X; Y) \) is high due to the strong dependencies among text tokens. This results in a higher likelihood of compounding error when tokens are generated in parallel. In contrast, as the timestep approaches zero, the mutual information between tokens conditioned on previously generated tokens \( Z \), denoted as \( I(X; Y \mid Z) \), decreases\footnote{
\( I(X; Y) \geq I(X; Y \mid Z) \) because conditioning on \( Z \) reduces the uncertainty about \( X \) and \( Y \), and \( Z \) may explain some of the shared information between them. For a more detailed discussion, please refer to the Appendix.}. Since \( Z \) reduces the mutual information between \( X \) and \( Y \), the error introduced by parallel token generation becomes negligible at these later timesteps.

Motivated by this observation, we thought that improving the sampling schedule to allocate more sampling steps in regions where the compounding error is larger could help reduce the compounding error. 


\jcc{I think the relation between Sec 3.1 and 3.2's result is not obvious. We need to clarify it (talk to you later)}
% \yh{Q: Should we explain this with more specific examples, e.g. 2d toy exmaple?}

\subsection{Estimating the Compounding Error Using Girsanov's Theorem}

\jc{which causes a mismatch between the inference and training distributions of the intermediate latents
produced during the parallel sampling process.}

As seen in Equation~\eref{equation:CDE}, estimating the compounding error requires computing the KL divergence between the true distribution and the approximated distribution. One effective method for computing the KL divergence between two stochastic processes is to use \textbf{Girsanov's theorem} \citep{ding2021markov, chen2022sampling}. A simplified version of Girsanov's theorem for two given time-inhomogeneous Continuous-Time Markov Chains (CTMCs) is as follows (proof provided in Appendix C):

\begin{theorem}
{
\normalfont{(KL-divergence Upper bound, KLUB)}} Consider the following two CTMCs: 
\[
    \begin{cases}
    
    \textrm { CTMC 1} : &  q^1_{t+dt|t}(y \mid x) = \delta_{xy} +R^1_t(x,y) dt + o(dt) \\ 
    \textrm { CTMC 2} : &  q^2_{t+dt|t}(y \mid x) = \delta_{xy} +R^2_t(x,y) dt + o(dt)  \end{cases}
    % \text { CTMC 1} : & \partial_t q^1_t(y \mid x) = R^1_t(x,y) dt + o(dt) \\ 
    % \text { CTMC 2} : & \partial_t q^2_t(y \mid x) = R^2_t(x,y) dt + o(dt)  \end{cases}
\]
Here, $\delta_{xy}$ refers to Dirac delta function, $R^1_t$ and $R^2_t$ represent the rate matrices of each CTMC, with a finite state space $S = \{x_1, \cdots, x_N\}$. Let $\mathbb{P}_T$ and $\mathbb{Q}_T$ be the resulting probability distributions at the time $T$ of the outputs of CTMC 1 and 2, respectively. 
\yh{If CTMC 1 and 2 start from the same initial distribution
\(\pi=\mathbb{P}_0=\mathbb{Q}_T\)}, then we have:
\begin{equation}
D_\mathrm{KL}(\mathbb{P}_T \| \mathbb{Q}_T) 
\le D_\mathrm{KL}(\mathbb{P}_{\text{paths}} \| \mathbb{Q}_{\text{paths}}) 
= 
\underbrace{\mathbb{E}_{\mathbb{P}_{\text{paths}}} \left[
\sum_{i,j} \sum_{\substack{0 < u \le T}} H_{u}^{ij} \log \frac{R^1_u(i,j)}{R^2_u(i,j)}
\right]}_{\mathclap{\textrm{\normalfont{KLUB}}(\mathbb{P}_T \| \mathbb{Q}_T)}} 
% = \mathbb{E}_{\mathbb{P}_{\text{paths}}} \left[
% \sum_{\substack{0 < u \le T}} H_{u}^{ij} \log ({R^1_u(i,j)}/{R^2_u(i,j)})
% \right]
\label{equation:KLUB}
\end{equation}
where \( \mathbb{P}_{\text{paths}} \) and \( \mathbb{Q}_{\text{paths}} \) denote the distributions over the path space \( \{ X_t \}_{t \in [0, T]} \), generated by CTMC 1 and CTMC 2, respectively. \(H_u^{ij}\) is an indicator function, where \( H_u^{ij} = 1 \) if a transition from state \( x_i \) to state \( x_j \) occurs at time \( u \); otherwise \( H_u^{ij} = 0 \).
\end{theorem}

We refer to the rightmost term in Equation~\eref{equation:KLUB} as the Kullback-Leibler divergence Upper Bound (KLUB). This value allows us to measure the mismatch between distributions generated by different continuous-time Markov chains (CTMCs) based on the differences in their rate matrices. Let us now consider CTMC 1 as the ground truth reverse CTMC, and CTMC 2 as the reverse CTMC with parallel sampling. The compounding error can be quantified as the KL divergence between the output distributions generated by the two CTMCs; therefore, the KLUB provides an upper bound for this error.

\yh{Q: Do we need this paragraph? $\shortto$} Notably, samplers that use parallel sampling can also be represented in the form of a CTMC. For example, in the case of \(\tau\)-leaping, the rate matrix is \yh{approximately} fixed as \( \tilde{R}'_u = \tilde{R}_t \) for \( u \in [t - \tau, t) \), where \( \tilde{R}' \) is the reverse rate matrix used by \(\tau\)-leaping and \( \tilde{R} \) is the ground truth reverse rate matrix at time \( t \). As a result, we can use the theorem above to quantify the compounding error of parallel sampling by computing the KLUB between the outputs of the exact reverse CTMC and the reverse CTMC using parallel sampling.

%%%%%%%%%%%%%%%%%%%%%%%
\jc{
---------------------------

As seen in Eq.~\eref{equation:CDE}, estimating the compounding error requires computing the KL divergence between the true distribution and the approximated distribution. One effective method for computing the KL divergence between two stochastic processes is to use \textbf{Girsanov's theorem} \citep{ding2021markov, chen2022sampling}. A simplified version of Girsanov's theorem for two given time-inhomogeneous Continuous-Time Markov Chains (CTMCs) is as follows (proof provided in Appendix C):

\begin{theorem}
{
\normalfont{(KL-divergence Upper bound, KLUB)}} Consider the following two CTMCs: 
\[
    \begin{cases}
    
    \textrm { CTMC 1} : &  q^1_{t+dt|t}(y \mid x) = \delta_{xy} +R^1_t(x,y) dt + o(dt) \\ 
    \textrm { CTMC 2} : &  q^2_{t+dt|t}(y \mid x) = \delta_{xy} +R^2_t(x,y) dt + o(dt)  \end{cases}
    % \text { CTMC 1} : & \partial_t q^1_t(y \mid x) = R^1_t(x,y) dt + o(dt) \\ 
    % \text { CTMC 2} : & \partial_t q^2_t(y \mid x) = R^2_t(x,y) dt + o(dt)  \end{cases}
\]
Here, $\delta_{xy}$ refers to Dirac delta function, $R^1_t$ and $R^2_t$ represent the rate matrices of each CTMC, with a finite state space $S = \{x_1, \cdots, x_N\}$. Let $\mathbb{P}_T$ and $\mathbb{Q}_T$ be the resulting probability distributions at the time $T$ of the outputs of CTMC 1 and 2, respectively. 
\yh{If CTMC 1 and 2 start from the same initial distribution
\(\pi=\mathbb{P}_0=\mathbb{Q}_T\)}, then we have:
\begin{equation}
D_\mathrm{KL}(\mathbb{P}_T \| \mathbb{Q}_T) 
\le D_\mathrm{KL}(\mathbb{P}_{\text{paths}} \| \mathbb{Q}_{\text{paths}}) 
= 
\underbrace{\mathbb{E}_{\mathbb{P}_{\text{paths}}} \left[
\sum_{i,j} \sum_{\substack{0 < u \le T}} H_{u}^{ij} \log \frac{R^1_u(i,j)}{R^2_u(i,j)}
\right]}_{\mathclap{\textrm{\normalfont{KLUB}}(\mathbb{P}_T \| \mathbb{Q}_T)}} 
% = \mathbb{E}_{\mathbb{P}_{\text{paths}}} \left[
% \sum_{\substack{0 < u \le T}} H_{u}^{ij} \log ({R^1_u(i,j)}/{R^2_u(i,j)})
% \right]
\label{equation:KLUB}
\end{equation}
where \( \mathbb{P}_{\text{paths}} \) and \( \mathbb{Q}_{\text{paths}} \) denote the distributions over the path space \( \{ X_t \}_{t \in [0, T]} \), generated by CTMC 1 and CTMC 2, respectively. \(H_u^{ij}\) is an indicator function, where \( H_u^{ij} = 1 \) if a transition from state \( x_i \) to state \( x_j \) occurs at time \( u \); otherwise \( H_u^{ij} = 0 \).
\end{theorem}

We refer to the rightmost term in Equation~\eref{equation:KLUB} as the Kullback-Leibler divergence Upper Bound (KLUB). This value allows us to measure the mismatch between distributions generated by different continuous-time Markov chains (CTMCs) based on the differences in their rate matrices. Let us now consider CTMC 1 as the ground truth reverse CTMC, and CTMC 2 as the reverse CTMC with parallel sampling. The compounding error can be quantified as the KL divergence between the output distributions generated by the two CTMCs; therefore, the KLUB provides an upper bound for this error.

\yh{Q: Do we need this paragraph? $\shortto$} Notably, samplers that use parallel sampling can also be represented in the form of a CTMC. For example, in the case of \(\tau\)-leaping, the rate matrix is \yh{approximately} fixed as \( \tilde{R}'_u = \tilde{R}_t \) for \( u \in [t - \tau, t) \), where \( \tilde{R}' \) is the reverse rate matrix used by \(\tau\)-leaping and \( \tilde{R} \) is the ground truth reverse rate matrix at time \( t \). As a result, we can use the theorem above to quantify the compounding error of parallel sampling by computing the KLUB between the outputs of the exact reverse CTMC and the reverse CTMC using parallel sampling.



}



\begin{theorem}
{
\normalfont{(KL-divergence Upper bound, KLUB)}} Consider the following two CTMCs: 
\[
    \begin{cases}
    
    \textrm { CTMC 1} : &  q^1_{t+dt|t}(y \mid x) = \delta_{xy} +R^1_t(x,y) dt + o(dt) \\ 
    \textrm { CTMC 2} : &  q^2_{t+dt|t}(y \mid x) = \delta_{xy} +R^2_t(x,y) dt + o(dt)  \end{cases}
    % \text { CTMC 1} : & \partial_t q^1_t(y \mid x) = R^1_t(x,y) dt + o(dt) \\ 
    % \text { CTMC 2} : & \partial_t q^2_t(y \mid x) = R^2_t(x,y) dt + o(dt)  \end{cases}
\]
Here, $\delta_{xy}$ refers to Dirac delta function, $R^1_t$ and $R^2_t$ represent the rate matrices of each CTMC, with a finite state space $S = \{x_1, \cdots, x_N\}$. \jc{Consider an interval of interest $[\alpha, \beta]$} Let $\mathbb{P}_\beta$ and $\mathbb{Q}_\beta$ be the resulting probability distributions at the time $t=\beta$ of the outputs of CTMC 1 and 2, respectively. 
\jc{If CTMC 1 and 2 start from the same initial distribution
\(\mathbb{P}_\alpha=\mathbb{Q}_\alpha\)}, then we have:
\begin{equation}
D_\mathrm{KL}(\mathbb{P}_\beta \| \mathbb{Q}_\beta) 
\le D_\mathrm{KL}(\mathbb{P}_{\text{paths}} \| \mathbb{Q}_{\text{paths}}) 
= 
\underbrace{\mathbb{E}_{\mathbb{P}_{\text{paths}}} \left[
\sum_{i,j} \sum_{\substack{\jc{\alpha < u \le \beta}}} H_{u}^{ij} \log \frac{R^1_u(i,j)}{R^2_u(i,j)}
\right]}_{\mathclap{\textrm{\normalfont{KLUB}}(\mathbb{P}_T \| \mathbb{Q}_T)}} 
\label{equation:KLUB}
\end{equation}
where \( \mathbb{P}_{\text{paths}} \) and \( \mathbb{Q}_{\text{paths}} \) denote the distributions over the path space \jc{\( \{ X_t \}_{t \in [\alpha, \beta]} \)}, generated by CTMC 1 and CTMC 2, respectively. \(H_u^{ij}\) is an indicator function, where \( H_u^{ij} = 1 \) if a transition from state \( x_i \) to state \( x_j \) occurs at time \( u \); otherwise \( H_u^{ij} = 0 \).
\end{theorem}


\subsection{Practical algorithm of KLUB estimation}

\yh{This section seems mathematically heavy. Do I need to move some derivation to the Appendix? $\downarrow$}

Using the KLUB derived above, we can formulate the sampling schedule optimization as a minimization problem. Starting with a simple case, suppose our sampling schedule is given by \((T, t, 0)\). Let \(\mathbb{Q}_0^{T \shortto t \shortto 0}\) represent the distribution generated by this schedule. Our objective is to find the optimal value of \(t\) that minimizes the compounding error. Restating our minimization problem, we aim to minimize the KLUB:

\begin{equation}
t^* = \argmin_{t\in(T,0)} \textrm{\normalfont{KLUB}}(
\mathbb{P}_0 \| \mathbb{Q}_0^{T \shortto t \shortto 0})
\label{equation:optimization}
\end{equation}
However, directly estimating \(\textrm{\normalfont{KLUB}}(\mathbb{P}_0 \| \mathbb{Q}_0^{T \shortto t \shortto 0})\) is practically infeasible. There are two main issues: First, sampling a single path \((X_u)_{u \in [T, 0]}\) under \(\mathbb{P}_{\text{paths}}\) is computationally expensive because it requires simulating the exact reverse CTMC from \(T\) to \(0\), which involves a high number of function evaluations (NFEs). Second, in the sampled trajectory \((X_u)_{u \in [T, 0]}\), only the transitions where \(H_{u}^{ij} = 1\) contribute to the expected value calculation in the KLUB. To obtain a reliable estimate, we need to compute the ratio of the rate matrices \( {R^1_u(i,j)}/{R^2_u(i,j)} \) for various \( i, j, u \). However, obtaining sufficient samples that cover all possible transitions across the state space and time is extremely challenging. To address this challenge, we employ two key techniques.

\paragraph{Technique 1: Maximizing KL Divergence from a Coarser Approximation}
Instead of minimizing the mismatch between the ground truth distribution \(\mathbb{P}_0\) and \(\mathbb{Q}_0^{T \shortto t \shortto 0}\), we opt to maximize the discrepancy between \(\mathbb{Q}_0^{T \shortto t \shortto 0}\) and a simpler, coarser approximation \(\mathbb{Q}_0^{T \shortto 0}\). The key insight is that by maximizing this divergence, we can identify the optimal sampling time \(t\) that indirectly minimizes the compounding error relative to the true distribution. Specifically, the relationship can be approximated as:

\[
D_\mathrm{KL}(\mathbb{Q}_0^{T\shortto t \shortto 0} \| \mathbb{Q}_0^{T\shortto 0})
\approx 
D_\mathrm{KL}(\mathbb{P}_0 \| \mathbb{Q}_0^{T\shortto 0})
- D_\mathrm{KL}(\mathbb{P}_0 \| \mathbb{Q}_0^{T\shortto t \shortto 0}),
\]

thus, maximizing the left-hand side divergence helps minimize the discrepancy \(D_\mathrm{KL}\big(\mathbb{P}_0 \,\big\|\, \mathbb{Q}_0^{T\shortto t \shortto 0}\big)\) between the true distribution \(\mathbb{P}_0\) and the optimized schedule \(\mathbb{Q}_0^{T\shortto t \shortto 0}\).

By comparing the two approximate distributions instead of the ground truth distribution, we reduce the sampling cost by sampling \((X_u)_{u \in [0, T]}\) under \(\mathbb{Q}_{\text{paths}}^{T \shortto t \shortto 0}\) instead of \(\mathbb{P}_{\text{paths}}\). Moreover, thanks to the fixed rate matrix under \(\tau\)-leaping, we can simplify the calculations significantly. Specifically:

\begin{subequations}
\begin{align}
\textrm{\normalfont{KLUB}}\big(\mathbb{Q}_0^{T\shortto t \shortto 0} \,\big\|\, \mathbb{Q}_0^{T \shortto 0}\big) 
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}} \left[
\sum_{u=0}^{T} H_{u}^{ij} \log 
\frac{R^{T\shortto t \shortto 0}_u(i,j)}{R^{T \shortto 0}_u(i,j)}
\right] \\
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}} \left[
\sum_{u=0}^{t} H_{u}^{ij} \log 
\frac{R_t(i,j)}{R_T(i,j)}
+ \sum_{u=t}^{T} H_{u}^{ij} 
\cancel{\log \frac{R_T(i,j)}{R_T(i,j)}}
\right] 
\label{equation:KLUB-coarse_to_fine-b}
\\
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}} \left[
\log \frac{R_t(i,j)}{R_T(i,j)} 
\sum_{u=0}^{t} H_{u}^{ij} 
\right]
\label{equation:KLUB-coarse_to_fine}
\end{align}
\end{subequations}

In \eref{equation:KLUB-coarse_to_fine-b}, we utilized the fact that under \(\tau\)-leaping, \(R^{T\shortto t \shortto 0}_u(i,j) = R_T(i,j)\) for \(u \in [t, T]\) and \(R^{T\shortto t \shortto 0}_u(i,j) = R_t(i,j)\) for \(u \in [0, t]\). In \eref{equation:KLUB-coarse_to_fine}, the rate matrices are constant over intervals, allowing us to pull \(\log \frac{R_t(i,j)}{R_T(i,j)}\) outside the summation.

\paragraph{Technique 2: Applying the Law of Total Expectation}

% Consider the meaning of \(\mathbb{E}\left[\sum_{u=0}^{t} H_{u}^{ij}\right]\); it calculates the expected number of transitions from state \(i\) to state \(j\) occurring between time \(0\) and \(t\). If we knew \(\partial_u p(x_u=j, x_{u-}=i)\), this could be found by \(\int_0^t \partial_u p(x_u=j, x_{u-}=i) \, du\). However, we do not have access to \(\partial_u p(x_u=j, x_{u-}=i)\).

Consider the meaning of \(\mathbb{E}\left[\sum_{u=0}^{t} H_{u}^{ij}\right]\); it calculates the average probability of a transition from \(i\) to \(j\) occurring between time \(0\) and \(t\). If we knew \(\partial_u p(x_u=j, x_{u-}=i)\), this could be found by \(\int_0^t \partial_u p(x_u=j, x_{u-}=i) \, du\). However, we do not have access to \(\partial_u p(x_u=j, x_{u-}=i)\).

Fortunately, we do know the conditional transition rate \(\partial_u p(x_u=j \mid x_{u-}=i) = R_t(i,j) \). Using this, we can rewrite \eref{equation:KLUB-coarse_to_fine}:

% Fortunately, we do know the conditional transition rate \(\partial_u p(x_u=j \mid x_{u-}=i) = R_t(i,j) \, du\). Using this, we can rewrite \eref{equation:KLUB-coarse_to_fine}:

\begin{subequations}
\begin{align}
\mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}}
\left[
\log \frac{R_t(i,j)}{R_T(i,j)} 
\sum_{t < u \leq T} H_{u}^{ij}
\right] 
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t}}
\left[
\mathbb{E}_{\mathbb{Q}_{\text{paths}}^{t \shortto 0}}
\left[
\log \frac{R_t(i,j)}{R_T(i,j)} \sum_{t < u \leq T} H_{u}^{ij} 
\Bigg| X_t = i\right]
\right] \label{equation:KLUB-simple-prev} \\
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t}}
\left[
\sum_{X_t\ne j}\log \frac{R_t(X_t,j)}{R_T(X_t,j)} \times R_t(X_t, j) \Delta t  
\right]
\label{equation:KLUB-simple}
\end{align}
\end{subequations}
Equation \eref{equation:KLUB-simple-prev} applies the Law of Total Expectation, and in \eref{equation:KLUB-simple}, we utilize the equation:
\[
\mathbb{E}_{\mathbb{Q}_{\text{paths}}^{t\shortto 0}}\left[ \log \frac{R_t(i,j)}{R_T(i,j)} \sum_{u=0}^{t} H_{u}^{ij} \Bigg| X_t = i\right] = \log \frac{R_t(i,j)}{R_T(i,j)} \times R_t(i,j) \Delta t,
\]
where \(\Delta t = t - 0 = t\).

In the original form of KLUB, Equation~\eref{equation:KLUB}, we needed to sample the ratio of rate matrices across \(i\), \(j\), and \(u\), but in Equation~\eref{equation:KLUB-simple}, sampling is only required over \(i\). This is because, given \(i\), we derived the expected value of the rate matrices ratio over \(j\) and \(u\) in closed form. The complete algorithm for KLUB computation combining Techniques 1 and 2 is provided in the Appendix.

Now, we can maximize \eref{equation:KLUB-simple}, using a standard optimization algorithm. Since we are dealing with a single variable \(t\), we employ the golden section search \citep{press2007numerical}, a well-known one-dimensional search algorithm, to find the value of \(t\) that maximizes the KLUB.

\subsection{Hierarchical Breakdown Strategy}

Up to this point, we have discussed how to decompose a coarse sampling schedule \((T, 0)\) into a finer sampling schedule \((T, t_1, 0)\) by finding an optimal intermediate timestep \( t_1 \). Now, we extend this approach to obtain sampling schedules with more steps. Our strategy is straightforward: we recursively split larger intervals into smaller ones, optimizing each new breakpoint to minimize the compounding error (see Figure X).

We begin with the coarsest sampling schedule \((T, 0)\) and use the golden section search to find the optimal \( t_1 \) that minimizes the KLUB. This refines the initial schedule into \((T, t_1, 0)\), effectively splitting the original interval into two parts.

Next, we further refine the sampling schedule into four intervals. We treat \((T, t_1)\) as a new coarse interval and find the optimal \( t_2 \) that maximizes the KLUB within this range, effectively splitting \((T, t_1)\) into \((T, t_2, t_1)\). We repeat the same process for the interval \((t_1, 0)\), finding the optimal \( t_3 \) that splits \((t_1, 0)\) into \((t_1, t_3, 0)\). After this step, the entire time range is divided into five timesteps: \((T, t_2, t_1, t_3, 0)\).

By repeating this process iteratively, we continue splitting each interval into two smaller intervals, each time optimizing the new breakpoint using the KLUB criterion. After \( K \) iterations, this hierarchical breakdown strategy yields a sampling schedule with \( 2^K \) NFEs, effectively optimizing the sampling schedule as the number of steps increases.

% So far, we have discussed how to decompose a coarse sampling schedule \((T, 0)\) into a finer sampling schedule \((T, t, 0)\). Now, let's extend this approach to more NFEs (Number of Function Evaluations). Our idea is straightforward: repeatedly split a large interval into two smaller intervals (Figure X). We start with the coarsest sampling schedule \((T, 0)\). Then, using the golden section search, we find the optimal \(t\). This refines the initial coarse sampling schedule into \((T, t_1, 0)\), effectively splitting the original interval into two parts. 

% Next, we aim to further refine the sampling schedule into four intervals. First, we treat \((T, t_1)\) as the new coarse interval and find the optimal \(t'_1\) that maximizes the KLUB within this range. We repeat the same process for the \((t_1, 0)\) interval. After this step, the entire time range is divided into four intervals: \((T, t_1, t_2, t_3, 0)\). By repeating this process iteratively, we continue splitting the time intervals. After \(K\) iterations, this hierarchical breakdown strategy will yield a sampling schedule corresponding to \(2^K\) NFEs, effectively optimizing the sampling schedule as the number of steps increases.

==> 3method_jesse.tex <==
\section{Optimizing the sampling schedule of discrete diffusion models}

For a fixed budget of sampling steps $n$, i.e., Number of Function Evaluation (NFE), our goal is to find an optimal sampling timestep \((T, t_1, \dots, t_n, 0)\) that minimizes the \textit{compounding decoding error} (CDE) caused by parallel sampling. In Section 3.1, we define and analyze the CDE, providing an intuitive understanding of how the sampling schedule is related to it. Next, we derive an upper bound on the CDE induced by parallel sampling (Section 3.2) and introduce techniques to compute the upper bound tractable and applicable for sampling schedule optimization (Section 3.3). Finally, in Section 3.4, we propose a hierarchical breakdown strategy that finds the optimal sampling schedule by decomposing a coarse schedule into finer steps. Although this section focuses on samplers based on \(\tau\)-leaping, all methods are also applicable to the \(k\)-Gillespie algorithm. For extensions to \(k\)-Gillespie, please refer to the Appendix.


\subsection{Motivating Examples: The Time-Dependent Nature of Compounding Errors}

\jc{We introduce a measure for the \emph{compounding decoding error} (CDE), $\mathcal E_{\mathrm{CDE}}$, which quantifies the discrepancy between the true joint distribution and the distribution obtained from parallel generation of different tokens. For demonstration, we consider a discrete process $\mathbf{X}_t = (X_t, Y_t, Z_t)$ with a sequence length of 3, consisting of tokens \( X_t \), \( Y_t \), and \( Z_t \). The general case is deferred to Appendix~\ref{}.}

% \yh{
% We propose measuring the CDE from $\mathbf{X}_s$ to $\mathbf{X}_t$ by using the KL divergence between the joint distribution \( P_{X_t,Y_t,Z_t|\mathbf{X}_s} \) and the product of marginal distributions \( P_{X_t|\mathbf{X}_s} \otimes P_{Y_t|\mathbf{X}_s} \otimes P_{Z_t|\mathbf{X}_s} \):
% \begin{equation}
% \mathcal E_{\mathrm{CDE}}(s \shortrightarrow t | \mathbf{X}_s) 
% \triangleq 
% \mathcal D_{\mathrm{KL}}(
% \underbrace{P_{X_t, Y_t, Z_t|\mathbf{X}_s}}_{\textrm{True distribution}} 
% \| 
% \underbrace{P_{X_t|\mathbf{X}_s} \otimes P_{Y_t|\mathbf{X}_s} \otimes P_{Z_t|\mathbf{X}_s} }_{\textrm{Approx.\ distribution from parallel sampling}} 
% ) 
% \label{equation:CDE}
% \end{equation}
% We note that the defined CDE is equivalent to the conditional mutual information \( \mathcal I(X_t; Y_t; Z_t | \mathbf{X}_s) \) of tokens \( X_t, Y_t, Z_t \):
% \[
% \mathcal E_{\mathrm{CDE}}(s \shortrightarrow t | \mathbf{X}_s) = \mathcal I(X_t; Y_t; Z_t  | \mathbf{X}_s).
% \]}

% \yh{This expression links the compounding error to mutual information between tokens; lower mutual information reduces parallel sampling error. In general, $\mathcal E_{\mathrm{CDE}}(t)$ varies over time based on the data distribution, corruption kernel (see Fig.~\ref{} for illustration), and DDM sampling methods.}

% Motivated by this observation, we will derive a tractable upper bound for $\mathcal E_{\mathrm{CDE}}(t)$ in the next section, depending on $t$. This allows us to allocate sampling timesteps in regions with higher CDE, thereby reducing the CDE — our strategy for optimizing sampling timesteps.

\jc{We propose measuring the CDE using the KL divergence between the joint distribution \( P_{X_t,Y_t,Z_t} \) and the product of marginal distributions \( P_{X_t} \otimes P_{Y_t} \otimes P_{Z_t} \) from parallel sampling:
\begin{equation}
\mathcal E_{\mathrm{CDE}}(t) 
\triangleq \mathcal D_{\mathrm{KL}}(
\underbrace{P_{X_t,Y_t, Z_t}}_{\textrm{True distribution}} 
\| 
\underbrace{P_{X_t} \otimes P_{Y_t} \otimes P_{Z_t} }_{\textrm{Approx.\ distribution from parallel sampling}} 
) 
\label{equation:CDE}
\end{equation}
We note that the defined CDE is equivalent to the mutual information \( I(X_t; Y_t; Z_t) \) of tokens \( X_t, Y_t, Z_t \):
\[
\mathcal E_{\mathrm{CDE}}(t) = \mathcal I(X_t; Y_t; Z_t).
\]

This expression links the compounding error to mutual information between tokens; lower mutual information reduces parallel sampling error. In general, $\mathcal E_{\mathrm{CDE}}(t)$ varies over time based on the data distribution, corruption kernel (see Fig.~\ref{} for illustration), and DDM sampling methods. 

Motivated by this observation, we will derive a tractable upper bound for $\mathcal E_{\mathrm{CDE}}(t)$ in the next section, depending on $t$. This allows us to allocate sampling timesteps in regions with higher CDE, thereby reducing the CDE — our strategy for optimizing sampling timesteps.}

% \begin{wrapfigure}{r}{6cm}
% \includegraphics[width=5cm]{figures-png/MI.png}
% \caption{
%     \textbf{MI.}
%     MI.
% }
% \label{homogenity-sample}
% \end{wrapfigure}

\subsection{Estimating the Compounding Error Using Girsanov's Theorem}



%%%%%%%%%%%%%%%%%%%%%%%
\jc{
As shown in \eref{equation:CDE}, computing $\mathcal{E}_{\mathrm{CDE}}(t)$ involves determining the KL divergence between the true distribution and the approximated distribution from DDM's parallel sampler, which is often intractable.

To address this, we treat the ground truth reverse process and the sampling process from DDM's parallel samplers (introduced in Sec.~\ref{}) as two CTMCs, starting from the same initial distribution. By applying \textbf{Girsanov's theorem}~\citep{ding2021markov, chen2022sampling}, we derive a tractable formula to compare the KL divergence between the distributions of these stochastic processes terminate at any time $t$. We summarize this as the following general theorem applicable to any two (forward/backward) CTMCs with $R^1_t$ and $R^2_t$ as their respective transition rate matrices:
\[
\begin{cases}
\textrm{CTMC 1}: & q^1_{t+dt|t}(y \mid x) = \delta_{xy} + R^1_t(x,y) dt + o(dt) \\ 
\textrm{CTMC 2}: & q^2_{t+dt|t}(y \mid x) = \delta_{xy} + R^2_t(x,y) dt + o(dt),
\end{cases}
\]
 We defer its proof to Appendix C.



\begin{theorem}
\normalfont{(KL-Divergence Upper Bound, KLUB)} 
Consider an interval $[\alpha, \beta]$. If both CTMCs start from the same initial distribution, $\mathbb{P}_\alpha = \mathbb{Q}_\alpha$, then we have:

\begin{equation}
\mathcal{D}_\mathrm{KL}(\mathbb{P}_\beta \| \mathbb{Q}_\beta) 
\le \mathcal{D}_\mathrm{KL}(\mathbb{P}_{\mathrm{paths}} \| \mathbb{Q}_{\mathrm{paths}}) 
= 
\underbrace{\mathbb{E}_{\mathbb{P}_{\mathrm{paths}}} \left[
\sum_{i,j} \sum_{\substack{\alpha < u \le \beta}} H_{u}^{ij} \log \frac{R^1_u(i,j)}{R^2_u(i,j)}
\right]}_{\triangleq~\textrm{\normalfont{KLUB}}(\mathbb{P}_\beta \| \mathbb{Q}_\beta)}. 
\label{equation:KLUB}
\end{equation}

Here, $\mathbb{P}_\beta$ and $\mathbb{Q}_\beta$ are the probability distributions at time $t$ resulting from CTMC 1 and CTMC 2, respectively. $\mathbb{P}_{\mathrm{paths}}$ and $\mathbb{Q}_{\mathrm{paths}}$ denote the distributions over their path spaces $\{ X_u \}_{u \in [\alpha, \beta]}$, generated by CTMC 1 and CTMC 2, respectively. The indicator function $H_u^{ij}$ is defined as $H_u^{ij} = 1$ if a transition from state $\rvx_i$ to state $\rvx_j$ occurs at time $u$, and $H_u^{ij} = 0$ otherwise.

\end{theorem}


We denote the rightmost term in \eref{equation:KLUB} as the \emph{Kullback-Leibler Divergence Upper Bound (KLUB)}, which quantifies the mismatch between distributions generated by different CTMCs based on their rate matrices. Consider CTMC 1 as the ground truth reverse CTMC and CTMC 2 as the reverse CTMC obtained via parallel sampling by substituting the forward transition kernel with the corresponding reverse-in-time kernel. Thus, $\mathcal{E}_{\mathrm{CDE}}(t)$ can be expressed as the KL divergence between the output distributions of the two CTMCs at time $t$, starting from the initial distribution $\pi$ at time $T$. This leads to the upper bound:
\begin{align*}
    \mathcal{E}_{\mathrm{CDE}}(t) \le \textrm{\normalfont{KLUB}}(\mathbb{P}_t \| \mathbb{Q}_t).
\end{align*}





\yh{Q: Do we need this paragraph? $\shortto$} Notably, samplers that use parallel sampling can also be represented in the form of a CTMC. For example, in the case of \(\tau\)-leaping, the rate matrix is \yh{approximately} fixed as \( \tilde{R}'_u = \tilde{R}_t \) for \( u \in [t - \tau, t) \), where \( \tilde{R}' \) is the reverse rate matrix used by \(\tau\)-leaping and \( \tilde{R} \) is the ground truth reverse rate matrix at time \( t \). As a result, we can use the theorem above to quantify the compounding error of parallel sampling by computing the KLUB between the outputs of the exact reverse CTMC and the reverse CTMC using parallel sampling.




\subsection{Coarse-to-Fine Timestep Searching Strategy}
Using the derived KLUB, we can formulate the timestep search as a minimization problem over KLUB. In a coarse-to-fine manner, suppose our sampling schedule is given by \((T, t, 0)\). Let \(\mathbb{Q}_0^{T \shortto t \shortto 0}\) represent the distribution generated by this schedule. Our goal is to find the optimal \(t\) that minimizes the CDE at time $0$ to match \(D_\mathrm{KL}(\mathbb{P}_0 \| \mathbb{Q}_0)\). This is approximately achievable by minimizing its KLUB upper bound:
\begin{equation}
t_1 \in \argmin_{t\in(T,0)} \textrm{\normalfont{KLUB}}(
\mathbb{P}_0 \| \mathbb{Q}_0^{T \shortto t \shortto 0})
\label{equation:optimization}
\end{equation}
With the initial refined interval \((T, t_1, 0)\), we seek optimal timesteps \(t_2 \in (T, t_1)\) and \(t_3 \in (t_1, 0)\) by solving the following minimization problems: 
\[
t_2 \in \argmin_{t\in(T,t_1)} \textrm{\normalfont{KLUB}}(
\mathbb{P}_{t_1} \| \mathbb{Q}_{t_1}^{T \shortto t \shortto t_1}) \quad \text{and} \quad t_3 \in \argmin_{t\in(t_1,0)} \textrm{\normalfont{KLUB}}(
\mathbb{P}_{0} \| \mathbb{Q}_{0}^{t_1 \shortto t \shortto 0}).
\] 
The first minimization problem targets matching \(D_\mathrm{KL}(\mathbb{P}_{t_1} \| \mathbb{Q}_{t_1})\), while the second focuses on matching \(D_\mathrm{KL}(\mathbb{P}_{0} \| \mathbb{Q}_{0})\).
This results in a further refined interval \((T, t_2, t_1, t_3, 0)\). By iterating this process, we continue splitting each interval into smaller ones, optimizing breakpoints using the KLUB criterion. After \(K\) iterations, this hierarchical strategy yields a sampling schedule with \(2^K\) NFEs, optimizing the schedule as the number of steps increases.

We visualize this recursive process of splitting larger intervals and optimizing each breakpoint to minimize CDE at these endpoints in Figure X.



}

\subsection{Practical algorithm of KLUB estimation}

\yh{This section seems mathematically heavy. Do I need to move some derivation to the Appendix? $\downarrow$}


However, directly estimating \(\textrm{\normalfont{KLUB}}(\mathbb{P}_0 \| \mathbb{Q}_0^{T \shortto t \shortto 0})\) is practically infeasible. There are two main issues: First, sampling a single path \((X_u)_{u \in [T, 0]}\) under \(\mathbb{P}_{\text{paths}}\) is computationally expensive because it requires simulating the exact reverse CTMC from \(T\) to \(0\), which involves a high number of function evaluations (NFEs). Second, in the sampled trajectory \((X_u)_{u \in [T, 0]}\), only the transitions where \(H_{u}^{ij} = 1\) contribute to the expected value calculation in the KLUB. To obtain a reliable estimate, we need to compute the ratio of the rate matrices \( {R^1_u(i,j)}/{R^2_u(i,j)} \) for various \( i, j, u \). However, obtaining sufficient samples that cover all possible transitions across the state space and time is extremely challenging. To address this challenge, we employ two key techniques.

\paragraph{Technique 1: Maximizing KL Divergence from a Coarser Approximation}
Instead of minimizing the mismatch between the ground truth distribution \(\mathbb{P}_0\) and \(\mathbb{Q}_0^{T \shortto t \shortto 0}\), we opt to maximize the discrepancy between \(\mathbb{Q}_0^{T \shortto t \shortto 0}\) and a simpler, coarser approximation \(\mathbb{Q}_0^{T \shortto 0}\). The key insight is that by maximizing this divergence, we can identify the optimal sampling time \(t\) that indirectly minimizes the compounding error relative to the true distribution. Specifically, the relationship can be approximated as:

\[
D_\mathrm{KL}(\mathbb{Q}_0^{T\shortto t \shortto 0} \| \mathbb{Q}_0^{T\shortto 0})
\approx 
D_\mathrm{KL}(\mathbb{P}_0 \| \mathbb{Q}_0^{T\shortto 0})
- D_\mathrm{KL}(\mathbb{P}_0 \| \mathbb{Q}_0^{T\shortto t \shortto 0}),
\]

thus, maximizing the left-hand side divergence helps minimize the discrepancy \(D_\mathrm{KL}\big(\mathbb{P}_0 \,\big\|\, \mathbb{Q}_0^{T\shortto t \shortto 0}\big)\) between the true distribution \(\mathbb{P}_0\) and the optimized schedule \(\mathbb{Q}_0^{T\shortto t \shortto 0}\).

By comparing the two approximate distributions instead of the ground truth distribution, we reduce the sampling cost by sampling \((X_u)_{u \in [0, T]}\) under \(\mathbb{Q}_{\text{paths}}^{T \shortto t \shortto 0}\) instead of \(\mathbb{P}_{\text{paths}}\). Moreover, thanks to the fixed rate matrix under \(\tau\)-leaping, we can simplify the calculations significantly. Specifically:

\begin{subequations}
\begin{align}
\textrm{\normalfont{KLUB}}\big(\mathbb{Q}_0^{T\shortto t \shortto 0} \,\big\|\, \mathbb{Q}_0^{T \shortto 0}\big) 
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}} \left[
\sum_{u=0}^{T} H_{u}^{ij} \log 
\frac{R^{T\shortto t \shortto 0}_u(i,j)}{R^{T \shortto 0}_u(i,j)}
\right] \\
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}} \left[
\sum_{u=0}^{t} H_{u}^{ij} \log 
\frac{R_t(i,j)}{R_T(i,j)}
+ \sum_{u=t}^{T} H_{u}^{ij} 
\cancel{\log \frac{R_T(i,j)}{R_T(i,j)}}
\right] 
\label{equation:KLUB-coarse_to_fine-b}
\\
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}} \left[
\log \frac{R_t(i,j)}{R_T(i,j)} 
\sum_{u=0}^{t} H_{u}^{ij} 
\right]
\label{equation:KLUB-coarse_to_fine}
\end{align}
\end{subequations}

In \eref{equation:KLUB-coarse_to_fine-b}, we utilized the fact that under \(\tau\)-leaping, \(R^{T\shortto t \shortto 0}_u(i,j) = R_T(i,j)\) for \(u \in [t, T]\) and \(R^{T\shortto t \shortto 0}_u(i,j) = R_t(i,j)\) for \(u \in [0, t]\). In \eref{equation:KLUB-coarse_to_fine}, the rate matrices are constant over intervals, allowing us to pull \(\log \frac{R_t(i,j)}{R_T(i,j)}\) outside the summation.

\paragraph{Technique 2: Applying the Law of Total Expectation}

% Consider the meaning of \(\mathbb{E}\left[\sum_{u=0}^{t} H_{u}^{ij}\right]\); it calculates the expected number of transitions from state \(i\) to state \(j\) occurring between time \(0\) and \(t\). If we knew \(\partial_u p(x_u=j, x_{u-}=i)\), this could be found by \(\int_0^t \partial_u p(x_u=j, x_{u-}=i) \, du\). However, we do not have access to \(\partial_u p(x_u=j, x_{u-}=i)\).

Consider the meaning of \(\mathbb{E}\left[\sum_{u=0}^{t} H_{u}^{ij}\right]\); it calculates the average probability of a transition from \(i\) to \(j\) occurring between time \(0\) and \(t\). If we knew \(\partial_u p(x_u=j, x_{u-}=i)\), this could be found by \(\int_0^t \partial_u p(x_u=j, x_{u-}=i) \, du\). However, we do not have access to \(\partial_u p(x_u=j, x_{u-}=i)\).

Fortunately, we do know the conditional transition rate \(\partial_u p(x_u=j \mid x_{u-}=i) = R_t(i,j) \). Using this, we can rewrite \eref{equation:KLUB-coarse_to_fine}:

% Fortunately, we do know the conditional transition rate \(\partial_u p(x_u=j \mid x_{u-}=i) = R_t(i,j) \, du\). Using this, we can rewrite \eref{equation:KLUB-coarse_to_fine}:

\begin{subequations}
\begin{align}
\mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t \shortto 0}}
\left[
\log \frac{R_t(i,j)}{R_T(i,j)} 
\sum_{t < u \leq T} H_{u}^{ij}
\right] 
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t}}
\left[
\mathbb{E}_{\mathbb{Q}_{\text{paths}}^{t \shortto 0}}
\left[
\log \frac{R_t(i,j)}{R_T(i,j)} \sum_{t < u \leq T} H_{u}^{ij} 
\Bigg| X_t = i\right]
\right] \label{equation:KLUB-simple-prev} \\
&= \mathbb{E}_{\mathbb{Q}_{\text{paths}}^{T\shortto t}}
\left[
\sum_{X_t\ne j}\log \frac{R_t(X_t,j)}{R_T(X_t,j)} \times R_t(X_t, j) \Delta t  
\right]
\label{equation:KLUB-simple}
\end{align}
\end{subequations}
Equation \eref{equation:KLUB-simple-prev} applies the Law of Total Expectation, and in \eref{equation:KLUB-simple}, we utilize the equation:
\[
\mathbb{E}_{\mathbb{Q}_{\text{paths}}^{t\shortto 0}}\left[ \log \frac{R_t(i,j)}{R_T(i,j)} \sum_{u=0}^{t} H_{u}^{ij} \Bigg| X_t = i\right] = \log \frac{R_t(i,j)}{R_T(i,j)} \times R_t(i,j) \Delta t,
\]
where \(\Delta t = t - 0 = t\).

In the original form of KLUB, Equation~\eref{equation:KLUB}, we needed to sample the ratio of rate matrices across \(i\), \(j\), and \(u\), but in Equation~\eref{equation:KLUB-simple}, sampling is only required over \(i\). This is because, given \(i\), we derived the expected value of the rate matrices ratio over \(j\) and \(u\) in closed form. The complete algorithm for KLUB computation combining Techniques 1 and 2 is provided in the Appendix.

Now, we can maximize \eref{equation:KLUB-simple}, using a standard optimization algorithm. Since we are dealing with a single variable \(t\), we employ the golden section search \citep{press2007numerical}, a well-known one-dimensional search algorithm, to find the value of \(t\) that maximizes the KLUB.


